Active Beam Learning for Full-Duplex Wireless Systems

In this paper, we present a novel active beam learning method for in-band full-duplex wireless systems, that aims to design transmit and receive beams which suppress self-interference and maximize the sum spectral efficiency. Rather than rely on explicit estimation of the downlink, uplink, and/or self-interference channels like in most existing work, our method instead actively probes all three channels through measurements of SNR and INR over a fixed number of time slots. Then, once this probing concludes, all collected probing measurements are used to design transmit and receive beams which serve downlink and uplink in a full-duplex fashion. We realize this active beam learning scheme through a network of LSTMs and DNNs, which learns to design each probing beam pair and subsequently extract and record valuable information from each probing measurement such that near-optimal serving beams can be designed following the probing stage. Simulation indicates that our method reliably suppresses self-interference while delivering near-maximal SNR on the downlink and uplink with merely 3-10 probing time slots, while exhibiting robustness to measurement noise and the structure of the self-interference channel.

==> alg/algorithm-solve-short.tex <==
\begin{algorithm}[!t]
\small
    \begin{algorithmic}[0]
        \REQUIRE $\thtxinit$, $\thrxinit$, $\inrrxthresh$, $\sesumtgt$, $\Delta\thetatx$, $\Delta\thetarx$, $\delta\thetatx$, $\delta\thetarx$ % $\parens{\deltatheta,\deltaphi}$, $\parens{\Delta\theta,\Delta\phi}$
        % \STATE $\sesummax = 0$ % , $\inrrxmin = \infty$
        % \STATE $\inrrxnom = \inrrx\thphtxrxijopt$
        \STATE $\txdirsetmeas = \thtxinit + \setnbr\parens{\Delta\thetatx,\delta\thetatx}$
        \STATE $\rxdirsetmeas = \thrxinit + \setnbr\parens{\Delta\thetarx,\delta\thetarx}$
        % \STATE $\set{V} = \txdirsetmeas \times \rxdirsetmeas$
        % \STATE $\set{D}_{\vartheta} = \braces{\Delta\vartheta = \maxop{\bars{\thetatx-\thetatx\idx{i\opt}},\bars{\thetarx-\thetarx\idx{j\opt}}} : \thphtx \in \txdirsetmeas\idx{i\opt}, \thphrx \in \rxdirsetmeas\idx{j\opt}}$
        \STATE $\set{D}_{\labeltx} = \braces{\Delta\varthetatx = \bars{\thetatx-\thtxinit}: \thtx \in \txdirsetmeas}$
        \STATE $\set{D}_{\labelrx} = \braces{\Delta\varthetarx = \bars{\thetarx-\thrxinit}: \thrx \in \rxdirsetmeas}$
        % \STATE $\set{D} = \braces{\Delta\vartheta^2 + \Delta\varphi^2 : \Delta\vartheta \in \set{D}_{\vartheta}, \Delta\varphi \in \set{D}_{\varphi}}$
        \STATE $\set{D} = \braces{\Delta\varthetatx^2 + \Delta\varthetarx^2 : \Delta\varthetatx \in \set{D}_{\labeltx}, \Delta\varthetarx \in \set{D}_{\labelrx}}$
        \STATE $\brackets{\sim,\set{J}} = \mathrm{sort}\parens{\set{D},\mathsf{ascend}}$
        % \STATE $\set{V} = \braces{\thphtxrx : \thphtx \in \txdirsetmeas\idx{i\opt}, \thphrx \in \rxdirsetmeas\idx{j\opt}}$
        % \STATE $\set{D} = \mathrm{sort}\parens{\txdirsetmeas\idx{i\opt} \times \rxdirsetmeas\idx{j\opt},\thphtxiopt,\thphrxjopt}$
        % \STATE $\sesummax = 0$
        \STATE Approximate (or measure) cross-link interference $\inrtx$.
        \STATE $\thtxopt = \thtxinit$, $\thrxopt = \thrxinit$, $\sesummax = 0$
        % \STATE $\thrxopt = \thrxinit$
        % \FOR{$\pthtxrx \in \entry{\set{V}}{\set{J}}$}
        \FOR{$\pthtxrx \in \entry{\txdirsetmeas \times \rxdirsetmeas}{\set{J}}$}
        % \FOR{$\parens{\thphtx,\thphrx} \in \txdirsetmeas\idx{i\opt} \times \rxdirsetmeas\idx{j\opt}$}
        \STATE Measure $\inrrx\thtxrx$  (or reference if already measured).
%        \IF{$\inrrx\thphtxrx < \inrrxmin$ and $\sesummax = 0$}
%        \STATE $\thphtxopt = \thphtx$
%        \STATE $\thphrxopt = \thphrx$
%        \IF{$\inrrx\thphtxrx \leq X$}
%        \STATE Break for-loop; \ginr target met; no further measurements required.
%        \ENDIF
%        \ENDIF
        \IF{$\inrrx\thtxrx \leq \inrrxtgt$}
        % \STATE Self-interference threshold met. % ; trigger a downlink and uplink quality check.
        % \STATE $\inrrxmin = \inrrx\thphtxrx$
        \STATE Measure (or reference) $\snrtx\pthtx$ and $\snrrx\pthrx$. % (or reference if measured).
        % \STATE Compute $\sinrtx\pthtx$ and $\sinrrx\pthtxrx$.
        \STATE $\sinrtx\pthtx = \snrtx\pthtx / \parens{1 + \inrtx}$
        \STATE $\sinrrx\pthtxrx = \snrrx\pthrx / \parens{1 + \inrrx\pthtxrx}$
        \STATE $\setx\pthtx = \logtwo{1 + \sinrtx\pthtx}$
        \STATE $\serx\pthtxrx = \logtwo{1 + \sinrrx\pthtxrx}$
        % \STATE Compute $\setx\pthtx$ and $\serx\pthtxrx$.
        \IF{$\setx\pthtx + \serx\pthtxrx > \sesummax$}
        \STATE $\pthtxrxopt = \pthtxrx$
        % \STATE $\thtxopt = \thtx$
        % \STATE $\thrxopt = \thrx$
        \STATE $\sesummax = \setx\pthtx + \serx\pthtxrx$
        \IF{$\sesummax \geq \sesumtgt$}
        \STATE Break for-loop; sum spectral efficiency target met. % ; no further measurements required.
        \ENDIF
        \ENDIF
        \ENDIF
        \ENDFOR
        \ENSURE $\thtxopt$, $\thrxopt$
    \end{algorithmic}
    \caption{Executing \steerp iteratively while collecting a reduced number of measurements.}
    \label{alg:algorithm-solve}
\end{algorithm}



==> alg/algorithm-solve.tex <==
\begin{algorithm}[!t]
    \begin{algorithmic}[0]
        \REQUIRE $\thtxinit$, $\thrxinit$, $\inrrxthresh$, $\sesumtgt$ % $\parens{\deltatheta,\deltaphi}$, $\parens{\Delta\theta,\Delta\phi}$
        % \STATE $\sesummax = 0$ % , $\inrrxmin = \infty$
        % \STATE $\inrrxnom = \inrrx\thphtxrxijopt$
        \STATE $\txdirsetmeas = \thtxinit + \setnbr\parens{\Delta\thetatx,\delta\thetatx}$
        \STATE $\rxdirsetmeas = \thrxinit + \setnbr\parens{\Delta\thetarx,\delta\thetarx}$
        % \STATE $\set{V} = \txdirsetmeas \times \rxdirsetmeas$
        % \STATE $\set{D}_{\vartheta} = \braces{\Delta\vartheta = \maxop{\bars{\thetatx-\thetatx\idx{i\opt}},\bars{\thetarx-\thetarx\idx{j\opt}}} : \thphtx \in \txdirsetmeas\idx{i\opt}, \thphrx \in \rxdirsetmeas\idx{j\opt}}$
        \STATE $\set{D}_{\labeltx} = \braces{\Delta\varthetatx = \bars{\thetatx-\thtxinit}: \thtx \in \txdirsetmeas}$
        \STATE $\set{D}_{\labelrx} = \braces{\Delta\varthetarx = \bars{\thetarx-\thrxinit}: \thrx \in \rxdirsetmeas}$
        % \STATE $\set{D} = \braces{\Delta\vartheta^2 + \Delta\varphi^2 : \Delta\vartheta \in \set{D}_{\vartheta}, \Delta\varphi \in \set{D}_{\varphi}}$
        \STATE $\set{D} = \braces{\Delta\varthetatx^2 + \Delta\varthetarx^2 : \Delta\varthetatx \in \set{D}_{\labeltx}, \Delta\varthetarx \in \set{D}_{\labelrx}}$
        \STATE $\brackets{\sim,\set{J}} = \mathrm{sort}\parens{\set{D},\mathsf{ascend}}$
        % \STATE $\set{V} = \braces{\thphtxrx : \thphtx \in \txdirsetmeas\idx{i\opt}, \thphrx \in \rxdirsetmeas\idx{j\opt}}$
        % \STATE $\set{D} = \mathrm{sort}\parens{\txdirsetmeas\idx{i\opt} \times \rxdirsetmeas\idx{j\opt},\thphtxiopt,\thphrxjopt}$
        % \STATE $\sesummax = 0$
        \STATE Approximate cross-link interference $\inrtx$ (or measure and feed back to the base station).
        \STATE $\thtxopt = \thtxinit$, $\thrxopt = \thrxinit$, $\sesummax = 0$
        % \STATE $\thrxopt = \thrxinit$
        % \FOR{$\pthtxrx \in \entry{\set{V}}{\set{J}}$}
        \FOR{$\pthtxrx \in \entry{\txdirsetmeas \times \rxdirsetmeas}{\set{J}}$}
        % \FOR{$\parens{\thphtx,\thphrx} \in \txdirsetmeas\idx{i\opt} \times \rxdirsetmeas\idx{j\opt}$}
        \STATE Measure (or reference) $\inrrx\thtxrx$.
%        \IF{$\inrrx\thphtxrx < \inrrxmin$ and $\sesummax = 0$}
%        \STATE $\thphtxopt = \thphtx$
%        \STATE $\thphrxopt = \thphrx$
%        \IF{$\inrrx\thphtxrx \leq X$}
%        \STATE Break for-loop; \ginr target met; no further measurements required.
%        \ENDIF
%        \ENDIF
        \IF{$\inrrx\thtxrx \leq \inrrxtgt$}
        \STATE Self-interference target met; trigger a DL and UL quality check.
        % \STATE $\inrrxmin = \inrrx\thphtxrx$
        \STATE Measure (or reference) $\snrtx\pthtx$ and $\snrrx\pthrx$.
        % \STATE Compute $\sinrtx\pthtx$ and $\sinrrx\pthtxrx$.
        \STATE $\sinrtx\pthtx = \snrtx\pthtx / \parens{1 + \inrtx}$
        \STATE $\sinrrx\pthtxrx = \snrrx\pthrx / \parens{1 + \inrrx\pthtxrx}$
        \STATE $\setx\pthtx = \logtwo{1 + \sinrtx\pthtx}$
        \STATE $\serx\pthtxrx = \logtwo{1 + \sinrrx\pthtxrx}$
        % \STATE Compute $\setx\pthtx$ and $\serx\pthtxrx$.
        \IF{$\setx\pthtx + \serx\pthtxrx > \sesummax$}
        \STATE $\thtxopt = \thtx$, $\thrxopt = \thrx$
        % \STATE $\thrxopt = \thrx$
        \STATE $\sesummax = \setx\pthtx + \serx\pthtxrx$
        \IF{$\sesummax \geq \sesumtgt$}
        \STATE Break for-loop; sum spectral efficiency target met; no further measurements required.
        \ENDIF
        \ENDIF
        \ENDIF
        \ENDFOR
        \ENSURE $\thtxopt$, $\thrxopt$
    \end{algorithmic}
    \caption{Executing \steerp iteratively while collecting a reduced number of measurements.}
    \label{alg:algorithm-solve}
\end{algorithm}
